Swift Markov Logic for Probabilistic Reasoning on Knowledge Graphs

We provide a framework for probabilistic reasoning in Vadalog-based Knowledge Graphs (KGs), satisfying the requirements of ontological reasoning: full recursion, powerful existential quantification, expression of inductive definitions. Vadalog is a Knowledge Representation and Reasoning (KRR) language based on Warded Datalog+/-, a logical core language of existential rules, with a good balance between computational complexity and expressive power. Handling uncertainty is essential for reasoning with KGs. Yet Vadalog and Warded Datalog+/- are not covered by the existing probabilistic logic programming and statistical relational learning approaches for several reasons, including insufficient support for recursion with existential quantification, and the impossibility to express inductive definitions. In this work, we introduce Soft Vadalog, a probabilistic extension to Vadalog, satisfying these desiderata. A Soft Vadalog program induces what we call a Probabilistic Knowledge Graph (PKG), which consists of a probability distribution on a network of chase instances, structures obtained by grounding the rules over a database using the chase procedure. We exploit PKGs for probabilistic marginal inference. We discuss the theory and present MCMC-chase, a Monte Carlo method to use Soft Vadalog in practice. We apply our framework to solve data management and industrial problems, and experimentally evaluate it in the Vadalog system. Under consideration in Theory and Practice of Logic Programming (TPLP).

==> script/artificial <==
#!/opt/local/bin/gnuplot
reset
set terminal pngcairo
set output '../10059313btzvytqdkmng/figures/artificial.png'
set grid
set autoscale
set title "(a) Execution time real-world settings" font ",18"
#set xlabel 'setting' font ",14"
set key top right
set style data histograms
set xtics offset 0.0,-0.35 font ",16"
set ytics font ",16"
#set ylabel 'Time (min:sec)' font ",16"
set ydata time
set timefmt "%H:%M:%S"
set style histogram
set style fill   solid 1.00 border lt -1
set style histogram clustered gap 1 title textcolor lt -1
set yrange ['00:00:00' : '00:30:00']
show grid

plot "artificial.data" using 2:xtic(1) title columnheader,\
	 "artificial.data" using 3:xtic(1) title columnheader,\
	 	 "artificial.data" using 4:xtic(1) title columnheader,\
	 	 	 "artificial.data" using 5:xtic(1) title columnheader,\
	 	 	 	 "artificial.data" using 6:xtic(1) title columnheader

==> script/artificial_error <==
#!/opt/local/bin/gnuplot
reset
set terminal pngcairo
set output 'artificial_error.png'
set grid
set autoscale
set title "(c) Error rate real-world settings" font ",18"
#set xlabel 'setting' font ",14"
set key top right
set style data histograms
set xtics offset 0.0,-0.35 font ",16" font ",16"
set ytics font ",16"
set xrange [-0.5:4]
#set ylabel 'Error rate' font ",16"
set style histogram
set style fill   solid 1.00 border lt -1
set style histogram clustered gap 1 title textcolor lt -1
show grid


plot "artificial_error.data" using 2:xtic(1) linecolor 2 title columnheader,\
	 "artificial_error.data" using 3:xtic(1) linecolor 3 title columnheader,\
	 	 "artificial_error.data" using 4:xtic(1) linecolor 4 title columnheader,\
	 	 	 "artificial_error.data" using 5:xtic(1) linecolor 5 title columnheader

==> script/real <==
#!/opt/local/bin/gnuplot
reset
set terminal pngcairo
set output 'real.png'
set grid
set autoscale
set title "(b) Execution time synthetic settings" font ",18"
#set xlabel 'setting' font ",14"
set key top left
unset key
set style data histograms
set xtics rotate font ",13" offset 0,0.2 
#set ylabel 'Time (min:sec)' font ",16"
set ytics font ",16"
set ydata time
set timefmt "%H:%M:%S"
set yrange ['00:00:00' : '00:25:00']
set style histogram
set style fill   solid 1.00 border lt -1
set style histogram clustered gap 1 title textcolor lt -1
#set style line 12 lc rgb '#808080' lt 0 lw 1
set grid back ls 0
show grid

plot "real.data" using 2:xtic(1) title columnheader,\
	 "real.data" using 3:xtic(1) title columnheader,\
	 	 "real.data" using 4:xtic(1) title columnheader,\
	 	 	 "real.data" using 5:xtic(1) title columnheader#,\
#	 	 	 	 "real.data" using 6:xtic(1) title columnheader

==> script/real_error <==
#!/opt/local/bin/gnuplot
reset
set terminal pngcairo
set output 'real_error.png'
set grid
set autoscale
set title "(d) Error rate synthetic settings" font ",18"
#set xlabel 'setting' font ",14"
set key top left
set style data histograms
set xtics rotate font ",13" offset 0,0.2 
set ytics font ",16"
#set ylabel 'Error rate' font ",13"
#set ydata time
#set timefmt "%H:%M:%S"
#set yrange ['00:00:00' : '00:20:00']
set style histogram
set style fill   solid 1.00 border lt -1
set style histogram clustered gap 1 title textcolor lt -1
#set style line 12 lc rgb '#808080' lt 0 lw 1
set grid back ls 0
unset key
show grid

plot "real_error.data" using 2:xtic(1) linecolor 2 title columnheader,\
	 "real_error.data" using 3:xtic(1) linecolor 3 title columnheader,\
	 	 "real_error.data" using 4:xtic(1) linecolor 4 title columnheader,\
	 	 	 "real_error.data" using 5:xtic(1) linecolor 5 title columnheader
